A Comprehensive Analysis of Swarming-based Live Streaming to Leverage Client Heterogeneity

Due to missing IP multicast support on an Internet scale, over-the-top media streams are delivered with the help of overlays as used by content delivery networks and their peer-to-peer (P2P) extensions. In this context, mesh/pull-based swarming plays an important role either as pure streaming approach or in combination with tree/push mechanisms. However, the impact of realistic client populations with heterogeneous resources is not yet fully understood. In this technical report, we contribute to closing this gap by mathematically analysing the most basic scheduling mechanisms latest deadline first (LDF) and earliest deadline first (EDF) in a continuous time Markov chain framework and combining them into a simple, yet powerful, mixed strategy to leverage inherent differences in client resources. The main contributions are twofold: (1) a mathematical framework for swarming on random graphs is proposed with a focus on LDF and EDF strategies in heterogeneous scenarios; (2) a mixed strategy, named SchedMix, is proposed that leverages peer heterogeneity. The proposed strategy, SchedMix is shown to outperform the other two strategies using different abstractions: a mean-field theoretic analysis of buffer probabilities, simulations of a stochastic model on random graphs, and a full-stack implementation of a P2P streaming system.

==> sections/0_abstract.tex <==
\begin{abstract} 
%%<<<<<<< .mine
	%\tdGeneral{Here comes the abstract\ldots}
	% Common ground
	Due to missing IP multicast support on an Internet scale, over-the-top media streams are delivered with the help of overlays as used by content delivery networks and their peer-to-peer (P2P) extensions.
	In this context, mesh/pull-based swarming plays an important role either as pure streaming approach or in combination with tree/push mechanisms.
	%
	% Problem
	%While a number of works study data scheduling for swarming and propose sophisticated solutions for it, 
	However, the impact of realistic client populations with heterogeneous resources is not yet fully understood.
	%
	% Our answer
	In this paper, we contribute to closing this gap by %revisiting 
	mathematically analysing the most basic scheduling mechanisms \emph{latest deadline first} (LDF) and \emph{earliest deadline first} (EDF) in a continuous time Markov chain framework and combining them into a simple, yet powerful, mixed strategy to leverage inherent differences in client resources.
	The contribution of this paper is, hence,  twofold: %threefold: 
	(1) a mathematical framework for swarming on random graphs is proposed with a focus on LDF and EDF strategies in heterogeneous  scenarios;
	%(2) LDF and EDF are extensively studied in heterogeneous scenarios;
	(2) a mixed strategy, named \sys{SchedMix}, is proposed that leverages peer heterogeneity.
	The proposed strategy, \sys{SchedMix} is shown to outperform the other two strategies using different abstractions: a mean-field theoretic analysis of buffer probabilities, simulations of a stochastic model on random graphs, and a full-stack implementation of a P2P streaming system.
	
	%%In this paper, we present a mathematical framework for peer-to-peer live video streaming on random graphs and document rudimentary results. We study two popular chunk selection strategies, \viz, latest deadline first (LDF) and earliest deadline first (EDF). LDF is known to be an efficient strategy, but suffers from high startup latency. EDF, on the other hand, fares poorly with increasing peer size, but enjoys small startup latency. We propose a mixed strategy where strong peers play LDF and weak peers, EDF. We show that the mixed strategy outperforms both pure LDF and EDF strategies, and necessitates much smaller startup latency. We offer validation of our proposition at three different levels of abstraction: mean-field theoretic analysis of buffer probabilities, simulation of the stochastic model on random graphs and finally on a full-stack simulation model. 
	
	% Common ground
	
	%
	% Problem
	
	%
	% Our answer
	
%%=======
%%% Common ground
%%Due to missing IP multicast support on an Internet scale, over-the-top video streams are delivered with the help of overlays as used by content delivery networks and their peer-to-peer (P2P) extensions.
%%In this context, mesh/pull-based swarming plays an important role either as pure streaming approach or in combination with tree/push mechanisms.
%%%
%%% Problem
%%However, the impact of realistic client populations with heterogeneous resources is not yet fully understood.
%%%
%%% Our answer
%%In this paper, we contribute to closing this gap by mathematically analysing the most basic scheduling mechanisms \emph{latest deadline first} (LDF) and \emph{earliest deadline first} (EDF) in a continuous time Markov chain framework and combining them into a simple, yet powerful, mixed strategy to leverage inherent differences in client resources.
%%The contribution of this paper is twofold:%threefold: 
%%(1) a mathematical framework for swarming on random graphs is proposed with a focus on LDF and EDF in heterogeneous scenarios;
%%(2) a mixed strategy is proposed that leverages peer heterogeneity.
%%The proposed strategy is shown to outperform the two variants using different abstractions: a mean-field theoretic analysis of buffer probabilities, simulations of a stochastic model on random graphs, and a full-stack implementation of a P2P streaming system.
%%>>>>>>> .r764
\end{abstract}
